Distributed Coverage Hole Prevention for Visual Environmental Monitoring with Quadcopters via Nonsmooth Control Barrier Functions

This paper proposes a distributed coverage control strategy for quadcopters equipped with downward-facing cameras that prevents the appearance of unmonitored areas in between the quadcopters' fields of view (FOVs). We derive a necessary and sufficient condition for eliminating any unsurveilled area that may arise in between the FOVs among a trio of quadcopters by utilizing a power diagram, i.e. a weighted Voronoi diagram defined by radii of FOVs. Because this condition can be described as logically combined constraints, we leverage nonsmooth control barrier functions (NCBFs) to prevent the appearance of unmonitored areas among a team's FOV. We then investigate the symmetric properties of the proposed NCBFs to develop a distributed algorithm. The proposed algorithm can support the switching of the NCBFs caused by changes of the quadcopters composing trios. The existence of the control input satisfying NCBF conditions is analyzed by employing the characteristics of the power diagram. The proposed framework is synthesized with a coverage control law that maximizes the monitoring quality while reducing overlaps of FOVs. The proposed method is demonstrated in simulation and experiment.

==> text/9-biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/Funada_trim_T-RO_filt3.jpg}}]{Riku Funada}
%Riku Funada 
received the B.Eng., M.Eng., and Ph.D. degrees in control engineering from the Tokyo Institute of Technology in 2014, 2016, and 2019, respectively. From 2016 to 2019, he was a Research Fellow of the Japan Society for the Promotion of Science. He was a Postdoctoral Researcher with the Waseda University in 2019 and the University of Texas at Austin in 2020. Since 2021, he has been an Assistant Professor at the Department of Systems and Control Engineering, Tokyo Institute of Technology. His research interests include cooperative control of networked robotics and motion planning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/Maria_trim.jpg}}]{Mar\'ia Santos}
%Mar\'ia Santos 
received the B.S./M.S. degree in industrial engineering from the University of Vigo, Vigo, Spain, in 2013, and the M.S. and Ph.D. degrees in electrical and computer engineering from the Georgia Institute of Technology, Atlanta, GA, USA, in 2016 and 2020, respectively. She is currently a Postdoctoral Researcher with the Department of Mechanical and Aerospace Engineering at Princeton University, Princeton, NJ, USA. She conducts research in control theory and robotics, with a focus on multi-agent systems. Santos is the recipient of a Fulbright Scholarship in 2014 and of ``la Caixa" Foundation Fellowship in 2017.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/Maniwa_trim.jpg}}]{Ryuichi Maniwa}
%Ryuichi Maniwa 
received the B.Eng. degrees in control engineering from the Tokyo Institute of Technology in 2021. He is currently with the Department of Systems and Control Engineering, Tokyo Institute of Technology, Tokyo, Japan. His research interests include control of multi-agent systems and nonlinear control.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/junya_yamauchi_trim2.jpg}}]{Junya Yamauchi}
%Junya Yamauchi 
received the Ph.D. degree from Tokyo Institute of Technology in 2018. He was an assistant professor at Tokyo Institute of Technology from 2018 to 2020 and is currently an assistant professor at the University of Tokyo from 2020. His research interests include autonomy in multi-robot systems. He is a member of SICE and IEEE.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/masayuki_fujita_ipc_trim2.jpg}}]{Masayuki Fujita}
%Masayuki Fujita 
is a professor at the University of Tokyo and a professor emeritus at Tokyo Institute of Technology. He received the Dr. Eng. degree from Waseda University in 1987. His research interests include passivity-based control in robotics and robust control.
He was the IEEE Control Systems Society (CSS) Vice President Conference Activities and the President of the SICE, Japan. He is a recipient of the 2021 IEEE CSS Distinguished Member Award and the 2008 IEEE Transactions on Control Systems Technology Outstanding Paper Award. He is a Life Fellow of IEEE and a Fellow of SICE.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/Sampei_trim.jpg}}]{Mitsuji Sampei}
%Mitsuji Sampei 
received the B.Eng., M.Eng., and Dr.Eng. degrees in control engineering from Tokyo Institute of Technology in 1983, 1985 and 1987, respectively. From 1987 to 1993, he was a research associate and then an associate professor at Chiba University.   Since 1993, he has been with Tokyo Institute of Technology where he is currently a professor at the Department of Systems and Control Engineering. 
His current research interests include nonlinear system theory and robotics.  
He was IPC Chair of IEEE CCA2010, SICE 2011, IEEE CDC 2015. He was a president of Japan Association of Automatic Control (2022/2023).

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figs/biography/EgerstedtHeadshot_trim2.jpg}}]{Magnus Egerstedt}
%Magnus Egerstedt 
is the Dean of Engineering at the University of California, Irvine. Prior to UCI, he was on the faculty at the Georgia Institute of Technology. He received the M.S. degree in Engineering Physics and the Ph.D. degree in Applied Mathematics from the Royal Institute of Technology, and the B.A. degree in Philosophy from Stockholm University. Egerstedt is the President of the IEEE Control Systems Society, and he conducts research in control theory and robotics. He has received several teaching and research awards and is a Fellow of IEEE, IFAC, and the Royal Swedish Academy of Engineering Science.
\end{IEEEbiography}
